Choral: Object-Oriented Choreographic Programming

We present Choral, the first choreographic programming language based on mainstream abstractions. The key idea in Choral is a new notion of data type, which allows for expressing that data is distributed over different roles. We use this idea to reconstruct the paradigm of choreographic programming through object-oriented abstractions. Choreographies are classes, and instances of choreographies are objects with states and behaviours implemented collaboratively by roles. Choral comes with a compiler that, given a choreography, generates an implementation for each of its roles. These implementations are libraries in pure Java, whose types are under the control of the Choral programmer. Developers can then modularly compose these libraries in their own programs, in order to participate correctly in choreographies. Choral is the first incarnation of choreographic programming offering such modularity, which finally connects more than a decade of research on the paradigm to practical software development. The integration of choreographic and object-oriented programming yields other powerful advantages, where the features of one paradigm benefit the other in ways that go beyond the sum of the parts. The high-level abstractions and static checks from the world of choreographies can be used to write concurrent and distributed object-oriented software more concisely and correctly. We obtain a much more expressive choreographic language from object-oriented abstractions than in previous work. For example, object passing makes Choral the first higher-order choreographic programming language, whereby choreographies can be parameterised over other choreographies without any need for central coordination. Together with subtyping and generics, this allows Choral to elegantly support user-defined communication mechanisms and middleware.

==> preamble.tex <==

\makeatletter
\newcommand*{\installoption}[2][acmart]{
 \expandafter\newif\csname if#2\endcsname
 \@ifclasswith{#1}{#2}{
   \csname#2true\endcsname
 }{}
}
\newcommand*{\obeyoption}[2]{
 \csname if#2\endcsname\else\csname #1false\endcsname\fi
}
\newcommand*{\excludeoption}[2]{
 \csname if#2\endcsname\csname #1false\endcsname\fi
}
\makeatother

\installoption{appendix}
\installoption{submission}
\installoption{draft}
\installoption{showframe}
\obeyoption{showframe}{draft}

\usepackage{xparse}
\usepackage{etoolbox}
\usepackage{environ}

\makeatletter
\newcommand{\IfLabelExistsTF}[3]{\@ifundefined{r@#1}{#3}{#2}}
\newcommand{\IfLabelExistsT}[2]{\IfLabelExistsTF{#1}{#2}{}}
\newcommand{\IfLabelExistsF}[2]{\IfLabelExistsTF{#1}{}{#2}}
\newcommand{\IfDefTF}[3]{\@ifundefined{#1}{#3}{#2}}
\newcommand{\IfDefT}[2]{\IfDefTF{#1}{#2}{}}
\newcommand{\IfDefF}[2]{\IfDefTF{#1}{}{#2}}
\makeatother




\newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}

\usepackage{subfiles}
\usepackage{xr}
\usepackage{currfile}

\ifdefined\docroot\else
 \let\docroot\currfilepath
\fi

\newcommand\IfDocRootTF[2]{%
 \ifcurrfilepath{\docroot}{#1}{#2}%
}
\newcommand\IfDocRootT[1]{\IfDocRootTF{#1}{}}
\newcommand\IfDocRootF[1]{\IfDocRootTF{}{#1}}

\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{microtype}

\ifshowframe
\AtEndPreamble{%
 \usepackage{showframe}%
 \renewcommand*\ShowFrameColor{\color{black!50}}
 \renewcommand*\ShowFrameLinethickness{.5pt}
}
\fi

\usepackage[x11names,rgb,html]{xcolor}

\colorlet{textcolor}{.}
\newcommand\usecolor[2]{\begingroup%
  \colorlet{uc@saved}{.}
  \color{#1}#2\color{uc@saved}
\endgroup}
\newcommand\cboxed[2]{\begingroup%
  \colorlet{cb@saved}{.}%
  \color{#1}%
  \boxed{\color{cb@saved}#2}%
\endgroup}

\usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{positioning}
\usetikzlibrary{tikzmark}
\usepackage{graphicx}
\usepackage{pgfplots}

\usepackage[british]{babel}


\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{centernot}
\usepackage{scalerel}
\usepackage{stmaryrd}
\SetSymbolFont{stmry}{bold}{U}{stmry}{m}{n}
\usepackage{mathtools}


\makeatletter
\DeclareFontEncoding{LS2}{}{\@noaccents}
\makeatother
\DeclareFontSubstitution{LS2}{stix}{m}{n}

\DeclareSymbolFont{largesymbolsstix}{LS2}{stixex}{m}{n}

\DeclareMathDelimiter{\lbrbrak}{\mathopen}{largesymbolsstix}{"EE}{largesymbolsstix}{"14}
\DeclareMathDelimiter{\rbrbrak}{\mathclose}{largesymbolsstix}{"EF}{largesymbolsstix}{"15}

\allowdisplaybreaks

\usepackage{array}
\usepackage{xtab}
\usepackage{booktabs}
\usepackage{multicol}

\usepackage{float}
\usepackage{placeins}
\usepackage{wrapfig}

\usepackage[inline]{enumitem}

\usepackage{hyperref}
\usepackage{nameref}

\usepackage[capitalise,nameinlink,noabbrev]{cleveref}
\makeatletter
\newcommand{\customlabel}[4][0]{%
  \protected@write\@auxout{}{\string\newlabel{#3}{{#4}{\thepage}{#4}{#3}{}}}%
  \protected@write\@auxout{}{\string\newlabel{#3@cref}{{[#2][#1][#1]#4}{\thepage}}}%
}
\newcommand{\phantomlabel}[4][0]{%
  \customlabel[#1]{#2}{#3}{#4}%
  \hypertarget{#3}{}%
}
\newcommand{\crefv}[1]{%
  \begingroup\@cref@compressfalse\@cref@sortfalse\cref{#1}\endgroup%
}
\newcommand{\Crefv}[1]{%
  \begingroup\@cref@compressfalse\@cref@sortfalse\Cref{#1}\endgroup%
}
\newcommand{\crefabbrev}[1]{%
  \begingroup\@cref@abbrevtrue\cref{#1}\endgroup%
}
\makeatother

\AtEndPreamble{\hypersetup{
  final,
}}


\usepackage{proof-dashed}
\usepackage{prftree}

\newcommand{\rname}[1]{\ensuremath{\textsc{\MakeLowercase{#1}}}}
\newcommand{\rlabel}[2]{{%
  \customlabel{infrule}{#2}{#1}%
  \hypertarget{#2}{#1}}}
\crefname{infrule}{Rule}{rules}
\Crefname{infrule}{Rule}{Rules}


\AtEndPreamble{
  \theoremstyle{acmdefinition}
  \newtheorem{remark}[theorem]{Remark}
}

\crefname{proof}{proof of}{proofs of}
\Crefname{proof}{Proof of}{Proofs of}

\newcommand{\prooflabel}[2]{{%
  \customlabel{proof}{#2}{\cref*{#1}}%
  \hypertarget{#2}{}}}


\bibliographystyle{ACM-Reference-Format}
\citestyle{acmauthoryear}


\usepackage[
  disable,     %
  obeyFinal,   %
  textwidth=\marginparwidth,
  textsize=footnotesize,
  colorinlistoftodos,
  prependcaption
]{todonotes}
\newcommand{\unsure}[2][]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommand{\change}[2][]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommand{\info}[2][]{\todo[linecolor=cyan,backgroundcolor=cyan!25,bordercolor=cyan,#1]{#2}}
\newcommand{\improvement}[2][]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green,#1]{#2}}

\makeatletter
\if@todonotes@disabled
\else %
\paperwidth=\dimexpr \paperwidth + 6cm\relax
\oddsidemargin=\dimexpr\oddsidemargin + 3cm\relax
\evensidemargin=\dimexpr\evensidemargin + 3cm\relax
\marginparwidth=\dimexpr \marginparwidth + 3cm\relax
\AtBeginDocument{\todo{Disable todos before submission}}
\fi
\makeatother


\makeatletter
\def\new@acronym#1#2{\expandafter\def\csname#1\endcsname{{\upshape #2}\xspace}}
\def\new@acronymexp#1#2{\expandafter\def\csname#1@exp\endcsname{{#2}}}
\NewDocumentCommand{\newacronym}{o m o}{%
  \IfNoValueTF{#1}{\def\n{#2}}{\def\n{#1}}
  \new@acronym{\n}{#2}
  \IfNoValueF{#3}{\new@acronymexp{\n}{#3}}
}
\def\expandacronym#1{\csname#1@exp\endcsname}
\makeatother

\newacronym[lts]{LTS}[Labelled Transition System]

\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\cod}{cod}
\DeclareMathOperator{\img}{img}


\def\crel#1{\mathrel{\mathcal{#1}}}

\def\disjoint{\mathrel{\#}}

\let\defeq\triangleq
\edef\defiff{\stackrel{\triangle}{\iff}}

\makeatletter
\newcount\c@repeat@count
\newcommand{\crepeat}[2]{%
  \begingroup
  \c@repeat@count=\z@
  \@whilenum\c@repeat@count<#1\do{#2\advance\c@repeat@count\@ne}%
  \endgroup
}
\makeatother

\newenvironment{bnftable}[3][]
	{\par\vspace{\abovedisplayskip}\indent%
	  \sbox0{$#2 \Coloneqq {}$}%
	  \sbox1{$#3$}%
	  \begin{xtabular}{%
	      >{\raggedleft$}m{\wd0}<{$}%
	      >{\raggedright$#1\begingroup}m{\wd1}<{\endgroup$}%
	      >{\quad\it}l<{}}}
	{\end{xtabular}\vspace{\belowdisplayskip}\par\noindent}

\usepackage[normalem]{ulem}
\makeatletter
\def\cb#1#2#3{{\fboxsep=0pt\colorbox{#1}{\vphantom{\uline{#3}}#2{#3}}}}
\def\defann#1#2{%
	\expandafter\def\csname#1\endcsname{%
		\def\ann@####1{\hbox{#2{\ensuremath{####1}}}}%
		\def\ann@@####1{#2{####1}}%
		\@ifstar{\ann@}{\ann@@}%
	}}
\makeatother

\newcommand{\newtext}{\color{blue}}
\newcommand{\oldtext}{\color{black}}
\newcommand{\pleaseCheck}{\todo{Remove this comment when the new text has been checked.}}
\let\newtext\relax
\let\oldtext\relax


